Training Data Leakage Analysis in Language Models

Recent advances in neural network based language models lead to successful deployments of such models, improving user experience in various applications. It has been demonstrated that strong performance of language models comes along with the ability to memorize rare training samples, which poses serious privacy threats in case the model is trained on confidential user content. In this work, we introduce a methodology that investigates identifying the user content in the training data that could be leaked under a strong and realistic threat model. We propose two metrics to quantify user-level data leakage by measuring a model's ability to produce unique sentence fragments within training data. Our metrics further enable comparing different models trained on the same data in terms of privacy. We demonstrate our approach through extensive numerical studies on both RNN and Transformer based models. We further illustrate how the proposed metrics can be utilized to investigate the efficacy of mitigations like differentially private training or API hardening.

==> sections/avocado.tex <==
\subsection{Avocado dataset}
\label{sec:avocado}
\paragraph{Dataset} We use the Avocado dataset \citep{avocado2015} that contains 322k email correspondences of 413 users. We use the $80\%/20\%$ training/val set split. We emphasize that this is a dataset where the users are not independent (i.e. sensitive information related to both the company and the users such as names, positions, partner company names etc. are shared across communications). This is an interesting setting as it is related to businesses providing language models to enterprise customers using their data and it also provides important insights in terms of user-level privacy protection. 

\paragraph{Model} We use a two-layer LSTM model as the language model for the next-word prediction task. We set both the embedding dimension and LSTM hidden-representation size to 128. We use the Adam optimizer with the learning rate set to 1e-3 and batch size to 32. We fix the vocabulary to the most frequent 10k tokens in the training corpus (out of 95k tokens). 

In this experiment, we train the language model for 25 epochs and obtain one snapshot of the model at each epoch (around the first quarter of an epoch). We run the tab attack and investigate the results (i.e. our training data leakage analysis with sequences where user count in $\mathcal{D}$ is one) for each snapshot of the model. %We provide the result of the first snapshot as an example in Table \ref{table:avocado} of Appendix \ref{sec:a1}. 
Figure \ref{fig:avocado} shows the progress of the model performance and the tab attack statistics as the model is being trained for 25 epochs. 
\begin{figure*}[ht]
     \centering
     \begin{subfigure}{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/avocado1.png}
         \caption{}
         \label{fig:avocado1}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/avocado2.png}
         \caption{}
         \label{fig:avocado2}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/avocado3.png}
         \caption{}
         \label{fig:avocado3}
     \end{subfigure}
        \caption{Results of the experiment on the language model trained on Avocado dataset \citep{avocado2015}. Figure (a) presents the performance of the model with the perplexity on the train and validation set. Tab attack is performed at each epoch on a snapshot of the model. Figure (b) shows the histogram of the length of the unique sequences leaked by the model over 25 epochs. Figure (c) presents the perplexities of these unique sequences. The width of the bins are proportional to the number of sequences that appear in them at the corresponding perplexity. We excluded last 10 epochs in Figure (c) for the sake of visualization.}
        \label{fig:avocado}
\end{figure*}
We first note from Figure \ref{fig:avocado1} that the train and validation perplexities are close for the language model, indicating that the model is not overfitted. This is due to choosing a rather small capacity model (less than 3M parameters). Somewhat expectedly, we observe in Figure \ref{fig:avocado2} that the number of unique sequences leaked by the model increases consistently as the model training continues (colors getting darker as we go right for each sequence length). Another interesting observation is that the majority of the unique sequences are having perplexities below 3 as the training continues. This unfortunately indicates that not returning any prediction when confidence is below a certain threshold may not be sufficient to provide privacy in some cases.

Looking at the individual unique sequences, we already see sensitive information such as names, names with positions, product specific information and partner company names being leaked by the model starting at epoch 2\footnote{Due to strict licensing requirements of the Avocado dataset, we are unable to provide specific examples. However, we present detailed results in the next experiment.}. We point out that the reason why unique sequences of such sensitive information can be leaked by the model even in the beginning of the training is that the user content is highly correlated. This means that the snippets of these unique sequences appear many times in the training data, although the particular order appears only once (e.g. the sequence $w_1, w_2, w_3, w_4$ being unique while 2-grams $w_1, w_2$ and $w_2, w_3$ and $w_3, w_4$ appearing many times). This causes the model to produce a long chain of correct predictions by learning parts of the connections from multiple users and the remaining few ones from a single user. Further observations of this experiment is presented below:
\begin{itemize}
    \item We believe that personally identifiable information (PII) scrubbing of the training data should be a crucial first step, especially if the user content is correlated, since choosing a small subset of the most frequent tokens does not disable the sensitive tokens to find their way into the vocabulary when they are repeated many times across users. Even when we fix the vocabulary with words appearing in at least 25 users' data (which hurts the utility substantially), we still observe sensitive tokens present in the vocabulary. Therefore, in general the ideal setting would be to have users as independent as possible and fixing the vocabulary after applying PII scrubbing with the tokens that appear among many users' data, instead of the most frequent ones, in case sensitive information might be repeated many times in a single user's data.
    \item We do not claim that any unique sequence leaked by the model would be a privacy concern. In fact, there are seemingly common sequences such as ``been able to do that" with the context ``... I have not" that happen to be unique for a user in the training data and the model provides the correct prediction\footnote{``been able to do" appears 13 times and ``to do that" appears 36 times in the data. The text has been altered to comply with the Avocado license.}. We note that this prediction may not be as surprising for a public model (i.e. low perplexity), therefore, it is possible to filter these cases further by comparing with a public model in perplexities. 
    \item We try the idea of not returning any prediction when the perplexity is above a certain threshold (i.e. the model does not have high confidence). Choosing the threshold as 8, the accuracy of the snapshot at the last epoch on the validation set drops from 28.29\% to 26.19\%. This had only a little effect while leaving many of the unique sequences with sensitive information untouched. Taking things to extremes, setting the threshold as 3 using the model snapshot at epoch 5 returns no unique sequences, but with an accuracy of 14.81\%. We believe that this technique along with a vocabulary fixed with the suggested principles above could potentially find better privacy-utility tradeoffs.
\end{itemize}
